Hybrid System Modelling and Simulation with Dirac Deltas

For a wide variety of problems, creating detailed continuous models of (continuous) physical systems is, at the very least, impractical. Hybrid models can abstract away short transient behaviour (thus introducing discontinuities) in order to simplify the study of such systems. For example, when modelling a bouncing ball, the bounce can be abstracted as a discontinuous change of the velocity, instead of resorting to the physics of the ball (de-)compression to keep the velocity signal continuous. Impulsive differential equations can be used to model and simulate hybrid systems such as the bouncing ball. In this approach, the force acted on the ball by the floor is abstracted as an infinitely large function in an infinitely small interval of time, that is, an impulse. Current simulators cannot handle such approximations well due to the limitations of machine precision. In this paper, we explore the simulation of impulsive differential equations, where impulses are first class citizens. We present two approaches for the simulation of impulses: symbolic and numerical. Our contribution is a theoretically founded description of the implementation of both approaches in a Causal Block Diagram modelling and simulation tool. Furthermore, we investigate the conditions for which one approach is better than the other.

==> experiment.tex <==
\section{Experiment: Bouncing Ball}

\subsection{Physical Model}

A free falling ball, with no friction, is governed by the following ordinary differential equation:
\begin{aligneq}\label{eq:bouncing_ball_ct_der}
\dert{v(t)} &= -g \\
\dert{y(t)} &= v(t) \\
\end{aligneq}

Momentum conservation allows us to abstract what happens during the moment of collision, and give us the velocity of the ball after the collision:
$$
v(t_0+\epsilon) = - v(t_c - \epsilon)
$$
where $t_0$ is the time of the collision, $\epsilon$ is an infinitely small constant, and the mass of the ball is assumed to be 1.

For the bouncing ball, the use of Dirac delta provide a compact notation to represent the model as an impulsive differential equation \shortcite{Corwin2008}:
\begin{aligneq}\label{eq:bouncing_ball_ct_der_imp}
\dert{v(t)} &= -g + \sum_{i=0} -2 v(t_i - \epsilon) \delta(t-t_i) \\
\dert{y(t)} &= v(t) \\
\end{aligneq}
\noindent where:\\
$t_i$ denotes a time of the collision;\\
$v(t_i - \epsilon)$ denotes the speed of the ball immediately before the collision;\\
$- 2 v(t_i - \epsilon)$ represents the change in the speed of the ball, cause by the impulse occurring at time $t_i$, that is $v(t_0+\epsilon) - v(t_c - \epsilon) = - 2v(t_c - \epsilon)$; \\ 

Normally, \cref{eq:bouncing_ball_ct_der_imp} can be solved analytically by splitting the time continuum into open intervals and defining the appropriate initial values.
For example, if the initial values are $y(0)=10$ and $v(0)=0$, then, in the interval $t \in (0, t_0)$ the trajectory of the ball is given by \cref{eq:bouncing_ball_ct_der} which can be easily solved. $t_0$ can be found by solving $y(t_0)=0$.
In the interval $t \in (t_0, t_1)$, the initial values are $y(0)=0$ and $v(t_1+\epsilon) = -v(t_1-\epsilon)$, and the solution is again given by \cref{eq:bouncing_ball_ct_der}. 

The current example is simple enough to be solved analytically. For most cases in practice, the impulsive differential equations can be non-linear, and simulation is used to observe the behavior.

\subsection{CBD Model}

\cref{fig:bouncing_ball} shows the CBD of the bouncing ball.
The Ball CBD represents the ball dynamics in free fall, assuming no friction and constant gravitational acceleration. When collisions occur, an impulse occurs, as in \cref{eq:bouncing_ball_ct_der_imp}.
In CBDs, this impulse is generated when the derivative of a discontinuity is performed. The CollisionDetector emits a discontinuity from 0 to 1, when the position of the ball $y$ crosses the 0 threshold.
The ImpulseCalculator essentially performs the derivative of the signal coming from the CollisionDetector (represented by the RisingEdge block), which is an impulse when a collision is detected, and multiplies that with $-2v$.

Arround the point of a single collision, the model represents the following equations:
\begin{aligneq}\label{eq:bouncing_ball_ct}
a(t) &= \frac{I(t) - m g}{m} \\
v(t) &= \int_0^t a(u) du + v(0) \\
y(t) &= \int_0^t v(u) du + y(0) \\
c(t) &= \conditional{1}{0}{y(t) \leq 0} \\
I(t) &= -2 v(t) \dert{c(t)}
\end{aligneq}
\noindent where: \\
$I(t)$ is the impulsive force;\\
$a(t)$ is the total acceleration imposed on the ball;\\
$v(t)$ is the velocity of the ball;\\
$c(t)$ is the output of the CollisionDetector block; \\
$m=1$ is the mass of the ball;

\cref{eq:bouncing_ball_ct}, for the purposes of simulation, is approximated by:
\begin{aligneq}\label{eq:bouncing_ball_dt}
a(t) &= \frac{I(t) - m g}{m} \\
v(t) &= v(t-h) + a(t-h)h \\
y(t) &= y(t-h) + v(t-h)h \\
c(t) &= \conditional{1}{0}{y(t) \leq 0} \\
I(t) &= -2 v(t) \frac{c(t) - c(t-h)}{h}
\end{aligneq}
\noindent where \\
$h < 1$ is the discretization factor; \\ 
$v(0) = 0$ is the initial speed; \\ 
$y(0) = 10$ is the initial position;

By inspecting \cref{eq:bouncing_ball_ct}, one notes that a collision only has an effect on the ball at the next time step.
This is a common assumption and the other approach, i.e., use the values $a(t)$ and $v(t)$ to approximate $v(t)$ and $y(t)$, respectively, lead to an algebraic loop which can be solved at every point in time, expect when there is a collision.
This problem could be solved by using a different discretization approach for each of the integrals in \cref{eq:bouncing_ball_ct} but that is uncommon, may violate the modularity of CBDs, and still causes an algebraic loop.

For the first part of the analysis, suppose that \cref{fig:bouncing_ball} is simulated with a classical continuous time simulator, which supports discontinuity location.
Suppose that the collision occurs at time $t_c$. 
It follows that:
\begin{aligneq}\label{eq:collision_ball_dt}
a(t_c) &= -2 v(t_c) \frac{1}{h} - g \\
v(t_c+h) &= - v(t_c) - gh \\
\end{aligneq}

For a very small time step $h$, we get exactly what we wanted: the velocity of the ball is inverted in the collision.

No Dirac deltas where used in the previous example.
Now we describe the same model, using Dirac deltas.
Let $t_c$ be the time of the first collision with the floor.
Then the CBD model in \cref{fig:bouncing_ball} can be written as:
\begin{aligneq}\label{eq:bouncing_ball_ct_dirac}
a(t) &= \frac{I(t) - m g}{m} \\
v(t) &= \int_0^t a(u) du + v(0) \\
y(t) &= \int_0^t v(u) du + y(0) \\
c(t) &= \conditional{1}{0}{y(t) \leq 0} \\
I(t) &= -2 v(t) \delta(t-t_c)
\end{aligneq}
Noting that $\dert{c(t)} = 0 + \delta(t-t_c)$.

Following our implementation of the simulator with support for Dirac deltas, at the time arround the collision, the model in \cref{eq:bouncing_ball_ct_dirac} is discretized to:
\begin{aligneq}\label{eq:bouncing_ball_dt_dirac}
a(t_c) &= -2 v(t_c) \delta - g \\
v(t_c) &= v(t_c-h) - m g h \\
v(t_c + h) 	&= v(t_c) + \pargroup{- g}h - 2 v(t_c)
y(t_c) &= y(t_c-h) + v(t_c-h)h \\
I(t_c) &= -2 v(t_c) \delta
\end{aligneq}
Which is simplified to:
\begin{aligneq}
v(t_c + h) 	&= - v(t_c) - g h
\end{aligneq}
Exactly the same conclusion as \cref{eq:collision_ball_dt}.

This result is backed up by the numerical experiment, shown in \cref{fig:bouncing_ball_position}. In the plot, three solutions are shown: \\ 
$y_\text{ct}$ is the solution obtained via the classical CBD simulator;\\
$y_\text{imp}$ is the solution obtained with the CBD simulator with support for impulses;\\
$y_\text{analytic}$ is the analytic solution;

\begin{figure}[htb]
\begin{center}
  \includegraphics[width=\columnwidth]{imgs/bouncing_ball_position}
  \caption{Trajectory of the position of the ball.}
  \label{fig:bouncing_ball_position}
\end{center}
\end{figure}

The solutions $y_\text{ct}$ and $y_\text{imp}$ coincide perfectly.
This is confirmed by their norm, shown in \cref{fig:bouncing_ball_errors}.

\begin{figure}[htb]
\begin{center}
  \includegraphics[width=\columnwidth]{imgs/bouncing_ball_errors}
  \caption{Instantaneous squared errors.}
  \label{fig:bouncing_ball_errors}
\end{center}
\end{figure}

The benefit of the encoding of Dirac deltas in the simulator is that it minimizes the risk of overflows occurring.
In the bouncing ball example, the value $-2 v(t) \frac{c(t) - c(t-h)}{h}$ can be very big, whereas the version that supports Dirac deltas directly only stores the value $-2 v(t)$.


==> scsprocbib.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                            %
%     THESE COMMANDS ARE REQUIRED TO WORK WITH SCSPROC.BST TO MAKE BIBLIO    %
%                                                                            %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\makeatletter
\let\@internalcite\cite
%
\def\cite{\def\@citeseppen{-1000}%
    \def\@cite##1##2{(##1\if@tempswa , ##2\fi)}%
    \def\citeauthoryear##1##2##3{##1 ##3}\@internalcite}
\def\citeNP{\def\@citeseppen{-1000}%
    \def\@cite##1##2{##1\if@tempswa , ##2\fi}%
    \def\citeauthoryear##1##2##3{##1 ##3}\@internalcite}
\def\citeN{\def\@citeseppen{-1000}%
%  Pierre L'Ecuyer's fix for multiple cite bug
%  Added by Paul J Sanchez on 4 October 2001
%   \def\@cite##1##2{##1\if@tempswa , ##2)\else{)}\fi}%
%   \def\citeauthoryear##1##2##3{##1 (##3}\@citedata}
    \def\@cite##1##2{##1\if@tempswa, ##2)\else{}\fi}%
    \def\citeauthoryear##1##2##3{##1 (##3)}\@citedata}
\def\citeA{\def\@citeseppen{-1000}%
    \def\@cite##1##2{(##1\if@tempswa , ##2\fi)}%
    \def\citeauthoryear##1##2##3{##1}\@internalcite}
\def\citeANP{\def\@citeseppen{-1000}%
    \def\@cite##1##2{##1\if@tempswa , ##2\fi}%
    \def\citeauthoryear##1##2##3{##1}\@internalcite}
%
\def\shortcite{\def\@citeseppen{-1000}%
    \def\@cite##1##2{(##1\if@tempswa , ##2\fi)}%
    \def\citeauthoryear##1##2##3{##2 ##3}\@internalcite}
\def\shortciteNP{\def\@citeseppen{-1000}%
    \def\@cite##1##2{##1\if@tempswa , ##2\fi}%
    \def\citeauthoryear##1##2##3{##2 ##3}\@internalcite}
\def\shortciteN{\def\@citeseppen{-1000}%
%  Pierre L'Ecuyer's fix for multiple cite bug
%  Added by Paul J Sanchez on 2 September 2002
%  should have caught this last year...
%   \def\@cite##1##2{##1\if@tempswa , ##2)\else{)}\fi}%
%   \def\citeauthoryear##1##2##3{##2 (##3}\@citedata}
% Shane G. Henderson fix for extra right bracket at end of optional material June 8, 2005
%    \def\@cite##1##2{##1\if@tempswa, ##2)\else{}\fi}%
    \def\@cite##1##2{##1\if@tempswa, ##2\else{}\fi}%
    \def\citeauthoryear##1##2##3{##2 (##3)}\@citedata}
\def\shortciteA{\def\@citeseppen{-1000}%
    \def\@cite##1##2{(##1\if@tempswa , ##2\fi)}%
    \def\citeauthoryear##1##2##3{##2}\@internalcite}
\def\shortciteANP{\def\@citeseppen{-1000}%
    \def\@cite##1##2{##1\if@tempswa , ##2\fi}%
    \def\citeauthoryear##1##2##3{##2}\@internalcite}
%
\def\citeyear{\def\@citeseppen{-1000}%
    \def\@cite##1##2{(##1\if@tempswa , ##2\fi)}%
    \def\citeauthoryear##1##2##3{##3}\@citedata}
\def\citeyearNP{\def\@citeseppen{-1000}%
    \def\@cite##1##2{##1\if@tempswa , ##2\fi}%
    \def\citeauthoryear##1##2##3{##3}\@citedata}
%
% \@citedata and \@citedatax:
%
% Place commas in-between citations in the same \citeyear, \citeyearNP,
% \citeN, or \shortciteN command.
% Use something like \citeN{ref1,ref2,ref3} and \citeN{ref4} for a list.
%
\def\@citedata{%
    \@ifnextchar [{\@tempswatrue\@citedatax}%
                  {\@tempswafalse\@citedatax[]}%
}

\def\@citedatax[#1]#2{%
\if@filesw\immediate\write\@auxout{\string\citation{#2}}\fi%
  \def\@citea{}\@cite{\@for\@citeb:=#2\do%
    {\@citea\def\@citea{, }\@ifundefined% by Young
       {b@\@citeb}{{\bf ?}%
       \@warning{Citation `\@citeb' on page \thepage \space undefined}}%
{\csname b@\@citeb\endcsname}}}{#1}}%

% don't box citations, separate with ; and a space
% also, make the penalty between citations negative: a good place to break.
%
\def\@citex[#1]#2{%
\if@filesw\immediate\write\@auxout{\string\citation{#2}}\fi%
  \def\@citea{}\@cite{\@for\@citeb:=#2\do%
    {\@citea\def\@citea{, }\@ifundefined% by Young
       {b@\@citeb}{{\bf ?}%
       \@warning{Citation `\@citeb' on page \thepage \space undefined}}%
{\csname b@\@citeb\endcsname}}}{#1}}%

% (from apalike.sty)
% No labels in the bibliography.
%
\def\@biblabel#1{}
\makeatother

\newdimen\bibindent
\bibindent=.25in

% SEC: was \def\thebibliography#1{\section*{\refname\@mkboth
% SEC: was   {\uppercase{\refname}}{\uppercase{\refname}}}\list
\def\thebibliography#1{\section*{\refname}\list
   {}{\settowidth\labelwidth{[#1]}
   \leftmargin \bibindent
   \itemindent -\bibindent
   \listparindent \itemindent
	 \itemsep 4pt
   \parsep 0pt
   \usecounter{enumi}}
   \def\newblock{}
   \sloppy
   \sfcode`\.=1000\relax}


==> tagged_signals.tex <==
\section{Tagged Signals}
\label{sec:generalizedcbds_definitions}

We base our definitions in the work of Lee \emph{et al.} \cite{Lee2005} and Broman \emph{et al.} \cite{Broman2015}.
However, we adapt them to highlight generalized functions.

A tagged signal is a function:
$$
x: T \times N \to V \cup \left \{ \epsilon \right \}
$$
where, in this paper, we will assume $T$ as the non-negative real numbers $\mathbb{R}^{+}_0$, $N$ the non-negative integers $\mathbb{N}_0$, $V$ the real numbers $\mathbb{R}$, and $ \epsilon $ the absent value.
$T \times N$ is a totally ordered set with a lexicographic order.
$T$ represents the measurable time and $N$ stands for the micro steps.

Given a signal $x: T \times N \to V \cup \left \{ \epsilon \right \}$ and a $t \in T$, we define: 
\begin{compactitem}
\item the initial value as $x((t,0)) \in V \cup \left \{ \epsilon \right \}$;
\item the final micro step at time $t$ as the minimal $m_f^t$ such that, for all $m \in N$, $m > m_f^t$ implies that $ x((t,m))=x((t,m_f^t))$;
\item the final value at time $t$ as $x((t,m_f^t))$.
\end{compactitem}

Intuitively, the final value is the last interesting value at the time $t$ since, at any other later micro step, the signal remains the same.
%Notice that this does not say anything about the signal at some $t' > t$.
It is possible that the final micro step is not defined, meaning that the signal never stabilizes. If that is the case, we have a chattering Zeno signal. 
We assume that the signals are non-chattering Zeno.

Given a signal $x: T \times N \to V \cup \left \{ \epsilon \right \}$, we induce the following two signals:
\begin{compactitem}
\item initial value signal $x_i: T \to V \cup \left \{ \epsilon \right \}$, defined as $x_i(t) = x((t,0))$;
\item final value signal $x_f: T \to V \cup \left \{ \epsilon \right \}$, defined as $x_f(t) = x((t,m_f^t))$, where $m_f^t$ is the final micro step at time $t$;
\end{compactitem}

Given a signal $x: T \times N \to V \cup \left \{ \epsilon \right \}$, we can classify it as:
\begin{compactitem}
\item non-absent iff for all $t \in T$, $x_i(t) \neq \epsilon $
\item generalized continuous time iff it is non absent and for all $t \in T$, $x_i(t) = x_f(t)$;
\item continuous time iff $x$ is generalized continuous time and for all $t \in T$, $m_f^t=0$;
\item generalized piece-wise continuous time iff $x$ is non-absent and, given a discrete set $D \subseteq T$, for all $t \in T \setminus D$, $x_i(t) = x_f(t)$, and $x_i(t)$ is left continuous, and $x_f(t)$ is right continuous\footnote{As defined for normal functions over real numbers.}.
\item piece-wise continuous time signal iff $x$, given a discrete set $D \subseteq T$, $x$ is a generalized piece-wise continuous time signal, for all $t \in D$, $m_f^t = 1$, and for all $t \in T \setminus D$, $m_f^t = 0$.
\end{compactitem}

The difference between the continuous time signal (analogously, the piece-wise continuous signal) and the generalized continuous time signal (analogously, the generalized piece-wise continuous signal) is that the latter allows impulses:
$x((t,m))$ is an impulse iff $x((t,m)) \neq \epsilon $ and $0 < m < m_f^t$.
The piece-wise continuous time signal does not allow impulses, whereas the generalized does.

Because we will be using a digital computer to run simulations, we define the discretized equivalents of the above defined time signals.
Given a $x: T \times N \to V \cup \left \{ \epsilon \right \}$ and a countable set $T_d \subseteq T$:
\begin{compactitem}
\item $x$ is a generalized discrete time signal iff $x_i$ is absent except at points $t_d \in T_d$ and for all $t \in T$, $x_i(t) = x_f(t)$;
\item $x$ is a discrete time signal iff it is generalized discrete time and for all $t \in T$, $m_f^t=0$;
\item $x$ is a generalized piece-wise discrete time signal iff $x_i$ is absent except at points $t_d \in T_d$ and, given a discrete set $D \subseteq T_d$, for all $t \in T \setminus D$, $x_i(t) = x_f(t)$.
\item $x$ is a piece-wise discrete time signal iff, given a discrete set $D \subseteq T_d$, $x$ is a generalized piece-wise continuous time signal, for all $t \in D$, $m_f^t = 1$, and for all $t \in T_d \setminus D$, $m_f^t = 0$
\end{compactitem}

Figure~\ref{fig:sample_signals} shows two sample signals.

\begin{figure}[t]
\begin{center}
  \includegraphics[width=\columnwidth]{imgs/sample_signals}
  \caption{A piece-wise discrete time signal (left) and a generalized discrete time signal (right).}
  \label{fig:sample_signals}
\end{center}
\end{figure}

